Modeling Short-Range and Three-Membered Ring Structures in Lithium Borosilicate Glasses using Machine Learning Potential

Lithium borosilicate (LBS) glass is a prototypical lithium-ion conducting oxide glasses available for an all-solid state buttery. Nevertheless, the atomistic modeling of LBS glass using $ab$ $initio$ (AIMD) and classical molecular dynamics (CMD) simulations have critical limitations due to computational cost and inaccuracy in reproducing the glass microstructures, respectively. To overcome these difficulties, a machine-learning potential (MLP) was examined in this work for modeling LBS glasses using DeepMD. The glass structures obtained by this MLP possessed fourhold-coordinated boron ($^4$B) confirmed well with the experimental data and abundance of three-membered rings. The models were energetically more stable compared with those constructed with a functional force-field even though both the models included reasonable $^4$B. The results confirmed MLP to be superior to model the boron-containing glasses and address the inherent shortcomings of the AIMD and CMD. This study also discusses some limitations of MLP for modeling glasses.

==> defines.tex <==
%
% reset font for DS2100 workstation. 17 May 90
%
% FONTS (there are some in smart.tex too.)
\font\smcp=cmcsc10    %font of small-cap letters for references.
\font\bigtitle=cmbx10 scaled \magstep2 %font of big letters for titles.
\font\bigtitle=cmbx12 % font of big letters for titles.
%\font\fnoter=cmr7     % font for footnote ROMAN text.
%\font\fnotei=cmmi7    % font for footnote ITALIC text.

%\font\smcp=cmr8     at 10pt        % small-cap letters
\font\fnrom=cmr10   at 10truept    % footnote text ROMAN.
\font\fnita=cmti10  at 10truept    % footnote text ITALIC.
\font\fntyp=cmitt10 at 10truept    % footnote italic typewriter.
\font\fnmi=cmmi10   at 10truept    % footnote math ITALIC. 
\font\fnsy=cmsy10   at 10truept    % footnote math SYMBOL. 
\font\fnex=cmex10   at 10truept    % footnote math EXTENSION. 

% fonts for large math symbols
\font\bigcala=cmsy10 scaled\magstep1
\font\bigcalb=cmsy10 scaled\magstep2
\font\bigcalc=cmsy10 scaled\magstep3

% NOTES FOR USING ESOTERIC FONTS: need to use \hbox{} to enclose the
% esoteric fonts, otherwise we would get only the usual roman font.
%
% Blackboard fonts of math sets
%\font\bbf=msym10 scaled \magstep1

% The following are for Stanford version of TeX
%\font\smcp=amr8     at 10pt        % small-cap letters
%\font\fnrom=amr10   at 10truept    % footnote text ROMAN.
%\font\fnita=amti10  at 10truept    % footnote text ITALIC.
%\font\fntyp=amitt10 at 10truept    % footnote italic typewriter.
%\font\fnmi=ammi10   at 10truept    % footnote math ITALIC. 
%\font\fnsy=amsy10   at 10truept    % footnote math SYMBOL. 
%\font\fnex=amex10   at 10truept    % footnote math EXTENSION. 
%
% fonts for large math symbols
%\font\bigcala=amsy10 scaled\magstep1
%\font\bigcalb=amsy10 scaled\magstep2
%\font\bigcalc=amsy10 scaled\magstep3

%
%****************************************************************
% Definition of twelve point fonts, adapted from the tex macro
% file manmac.tex for the TeXbook by D. Knuth.  This file is 
% in directory /usr/local/lib/tex/inputs.
% vql, 26may90
%****************************************************************
%
% Font names for twelve point fonts from file lfonts.tex 
% see /usr/local/lib/tex/inputs/lfonts.tex
%
% twelve point
 \font\twlrm  = cmr12                 % roman  
 \font\twlmi  = cmmi12               % math italic
    \skewchar\twlmi ='177          %  for placement of accents
%\font\twlmib = cmmib10   \@magscale1 % bold math italic
%\font\twlsy  = cmsy10   \@magscale1 % math symbols
 \font\twlsy  = cmsy10    scaled\magstep1 % math symbols
    \skewchar\twlsy ='60           %   for placement of math accents
%\font\twlsyb = cmbsy10  \@magscale1 % bold symbols
 \font\twlit  = cmti12               % text italic
 \font\twlsl  = cmsl12               % slanted
 \font\twlbf  = cmbx12               % extended bold 
%\font\twlbfs = cmbxsl10 \@magscale1 % extended bold slanted
 \font\twltt  = cmtt12               % typewriter
    \hyphenchar\twltt = -1         %  suppress hyphenation in \tt font
%\font\twltti = cmitt10  \@magscale1 % italic typewriter
%\font\twltts = cmsltt10 \@magscale1 % slanted typewriter
 \font\twlsf  = cmss12               % sans serif
%\font\twlsfi = cmssi10  \@magscale1 % italic sans serif
%\font\twlsfb = cmssbx10 \@magscale1 % bold sans serif
%\font\twlsc  = cmcsc10  \@magscale1 % small caps
%\font\twlly  = lasy10  \@magscale1 % LaTeX symbols
%\font\twllyb = lasyb10 \@magscale1 % bold LaTeX symbols
%\font\twluit = cmu10    \@magscale1 % unslanted italic

%
% from manmac.tex
% see /usr/local/lib/tex/inputs/manmac.tex
%
\catcode`@=11 % borrow the private macros of PLAIN (with care)

\font\tentex=cmtex10

\font\inchhigh=cminch
\font\titlefont=cmssdc10 at 40pt

\font\ninerm=cmr9
\font\eightrm=cmr8
\font\sixrm=cmr6

\font\ninei=cmmi9
\font\eighti=cmmi8
\font\sixi=cmmi6
\skewchar\ninei='177 \skewchar\eighti='177 \skewchar\sixi='177

\font\ninesy=cmsy9
\font\eightsy=cmsy8
\font\sixsy=cmsy6
\skewchar\ninesy='60 \skewchar\eightsy='60 \skewchar\sixsy='60

\font\eightss=cmssq8

\font\eightssi=cmssqi8

\font\ninebf=cmbx9
\font\eightbf=cmbx8
\font\sixbf=cmbx6

\font\ninett=cmtt9
\font\eighttt=cmtt8

%% modifies March 26
%%
%%\hyphenchar\tentt=-1 % inhibit hyphenation in typewriter type
%%%%\hyphenchar\ninett=-1
%%\hyphenchar\eighttt=-1

\font\ninesl=cmsl9
\font\eightsl=cmsl8

\font\nineit=cmti9
\font\eightit=cmti8

\newskip\ttglue
\def\twlpoint{\def\rm{\fam0\twlrm}%
  \textfont0=\twlrm \scriptfont0=\ninerm \scriptscriptfont0=\sevenrm
  \textfont1=\twlmi \scriptfont1=\ninei \scriptscriptfont1=\seveni
  \textfont2=\twlsy \scriptfont2=\ninesy \scriptscriptfont2=\sevensy
  \def\it{\fam\itfam\twlit}%
  \textfont\itfam=\twlit
  \def\sl{\fam\slfam\twlsl}%
  \textfont\slfam=\twlsl
  \def\bf{\fam\bffam\twlbf}%
  \textfont\bffam=\twlbf \scriptfont\bffam=\ninebf
   \scriptscriptfont\bffam=\sevenbf
  \def\tt{\fam\ttfam\twltt}%
  \textfont\ttfam=\twltt
  \tt \ttglue=.5em plus.25em minus.15em
  \normalbaselineskip=14pt
  \def\MF{{\manual META}\-{\manual FONT}}%
  \let\sc=\tenrm
  \let\big=\tenbig
  \setbox\strutbox=\hbox{\vrule height8.5pt depth3.5pt width\z@}%
  \normalbaselines\rm}

\def\tenpoint{\def\rm{\fam0\tenrm}%
  \textfont0=\tenrm \scriptfont0=\sevenrm \scriptscriptfont0=\fiverm
  \textfont1=\teni \scriptfont1=\seveni \scriptscriptfont1=\fivei
  \textfont2=\tensy \scriptfont2=\sevensy \scriptscriptfont2=\fivesy
  \textfont3=\tenex \scriptfont3=\tenex \scriptscriptfont3=\tenex
  \def\it{\fam\itfam\tenit}%
  \textfont\itfam=\tenit
  \def\sl{\fam\slfam\tensl}%
  \textfont\slfam=\tensl
  \def\bf{\fam\bffam\tenbf}%
  \textfont\bffam=\tenbf \scriptfont\bffam=\sevenbf
   \scriptscriptfont\bffam=\fivebf
  \def\tt{\fam\ttfam\tentt}%
  \textfont\ttfam=\tentt
  \tt \ttglue=.5em plus.25em minus.15em
  \normalbaselineskip=12pt
  \def\MF{{\manual META}\-{\manual FONT}}%
  \let\sc=\eightrm
  \let\big=\tenbig
  \setbox\strutbox=\hbox{\vrule height8.5pt depth3.5pt width\z@}%
  \normalbaselines\rm}

\def\eightpoint{\def\rm{\fam0\eightrm}%
  \textfont0=\eightrm \scriptfont0=\sixrm \scriptscriptfont0=\fiverm
  \textfont1=\eighti \scriptfont1=\sixi \scriptscriptfont1=\fivei
  \textfont2=\eightsy \scriptfont2=\sixsy \scriptscriptfont2=\fivesy
  \textfont3=\tenex \scriptfont3=\tenex \scriptscriptfont3=\tenex
  \def\it{\fam\itfam\eightit}%
  \textfont\itfam=\eightit
  \def\sl{\fam\slfam\eightsl}%
  \textfont\slfam=\eightsl
  \def\bf{\fam\bffam\eightbf}%
  \textfont\bffam=\eightbf \scriptfont\bffam=\sixbf
   \scriptscriptfont\bffam=\fivebf
  \def\tt{\fam\ttfam\eighttt}%
  \textfont\ttfam=\eighttt
  \tt \ttglue=.5em plus.25em minus.15em
  \normalbaselineskip=9pt
  \def\MF{{\manual opqr}\-{\manual stuq}}%
  \let\sc=\sixrm
  \let\big=\eightbig
  \setbox\strutbox=\hbox{\vrule height7pt depth2pt width\z@}%
  \normalbaselines\rm}

%*******************************************************************

%
% fonts for footnotes
%
% old way
% define for 6pt baselineskip and roman font for footnote
%\def\fnsr{\sixspacing\fnrom}
% define for 6pt baselineskip and italic font for footnote
%\def\fnsi{\sixspacing\fnita}
% foonote fonts are just the family of ten-point fonts
\def\fnsr{\tenpoint\sixspacing}
% define for 6pt baselineskip and italic font for footnote
\def\fnsi{\tenpoint\sixspacing}

% DEFINES FOR LETTER LAYOUT
\def\begintabrag{\begingroup\parskip=0pt\parindent=0pt
		 \obeylines\advance\leftskip by}
\def\endtabrag{\endgroup}
%
% EXAMPLE:
% 
% \begintabrag 0.55\hsize
% August 17, 1990
% \endtabrag
% 
% \medskip
% \begintabrag 0pt
% Person in charge of addresses
% Editorial Office, {\it Mechanics of Materials}
% Department of A.M.E.S.
% University of California, San Diego
% La Jolla, CA 92093
% \endtabrag
% 
% \medskip
% \noindent To whom it may concern:
% 
% \medskip
% ... text ...
% 
% \medskip
% \begintabrag 0.55\hsize
% Yours sincerely
% \vskip 1 in
% Peter Mataga
% Assistant Professor
% \endtabrag
% 

% DEFINES FOR PAPER LAYOUT.

\def\clearpage{\vfill\eject}
\def\dsp{\displaystyle} % for math expressions in text.

%\def\endproof{\quad \vrule height 8pt width 4pt \rm} %end-proof mark
% end-proof mark
\def\endproof{\quad \hbox{\vrule height 8pt width 4pt} } 
% right-justified endproof mark
\def\rendproof{\hfill \endproof}
% Blank line with right-justified endproof mark
\def\lendproof{\line{\hfill \endproof}}

\def\hrulefill{\leaders\hrule height0.8pt\hfill} %fill with horiz line
\def\idone{\parindent=0 truein    %back-indenting by 1 truein
           \hangindent=1 truein \hangafter=1}
\def\idref{\parindent=0 truein    %back-indenting for references
           \hangindent=0.25 truein \hangafter=1}

% Set of integers: Z (character '132) in blackboard font
\def\integer{\hbox{\bbf \char'132}}

\def\leaderfill{\leaders \hbox to 1em{\hss.\hss}\hfill}
\def\leftendproof{\line{\hss\endproof}}
% defines for short lines
\def\sline{ \hbox{\vrule height 0.5 truept width 0.8 truein }} 
% the defines \litem and \ritem (and related defines) are from the 
% book on TeX (German), and not the same defines as in smartpc.tex
\def\litem{\par\noindent
               \hangindent=\parindent\ltextindent}
\def\ltextindent#1 {\hbox to \hangindent {#1 \hss}\ignorespaces}

% Set of natural numbers:
\def\natural{\hbox{\rm I\kern-0.2emN}} 

\def\ritem{\par\noindent\hangindent=-\parindent
           \hangafter=0
           \rtextindent}
\def\rtextindent#1{\hbox to 0pt{\hskip\hsize
                     \hbox to 0pt{\hss#1}\hss}%
                   \ignorespaces}
\def\pp{\hangindent=0.4 truein\hangafter=-1} %begin paragraph
\def\script{\scriptstyle}
\def\vuquoc{\hbox{Vu-Quoc\ }} %to prevent TeX to separate the name into
                     %two. Also add a space behind.

% definition of 'poor-man-bold' (TeXbook, p. 386)
% This is used mainly for lower-case Greek letters
\def\pmb#1{\setbox0=\hbox{#1}%
  \kern-.025em\copy0\kern-\wd0
  \kern.05em\copy0\kern-\wd0
  \kern-.025em\raise.0433em\box0 }
\def\pb #1{{\pmb{$#1$}}}

% defines of boldface for other letters 
\def\bold #1 { {\bf #1 } }
\def\b#1{{\bf #1}}

% Defines for Swedish, German: to put a circle on top of a letter.
\def\a#1{\accent'27#1}

% DEFINES FOR MATHEMATICAL EQUATIONS.

% defines for having more blank space between lines in a matrix
\def\blkl{\vphantom{\int\limits_a^a}}

% Dot product
% PC version 
%\def\dotprod{\hbox{\raise.5ex \hbox{\Largebf .} }}
%
\def\dotprod{\hbox{\raise.5ex \hbox{\textfont2=\sixsy $\,\bullet$} }}

% dot and circle for small letters
% to have "u big dot" just type {\d u}

% PC version
% similarly for "u with two circles" type {\cc u}, and so on...
%\def\d#1{{\vbox{\baselineskip=0.09truein \lineskiplimit=0pt 
%\moveright0.02truein\hbox{\Largebf .}\hbox{$#1$}}}}
%\def\dd#1{{\vbox{\baselineskip=0.09truein \lineskiplimit=0pt 
%\hbox{\hbox{\largebf .}\hbox{\kern-0.1em \largebf .}}
%\hbox{$#1$\lower0.3ex \hbox{}} }}}

\def\d#1{{\vbox{\baselineskip=0.09truein \lineskiplimit=0pt 
\moveright0.02truein\hbox{\textfont2=\sixsy $\bullet$}\hbox{$#1$}}}}
\def\cc#1{{\vbox{\baselineskip=0.09truein \lineskiplimit=0pt 
\hbox{\hbox{\fiverm o}\hbox{\fiverm o}}\hbox{$#1$}}}}
\def\dd#1{{\vbox{\baselineskip=0.09truein \lineskiplimit=0pt 
\hbox{\hbox{\textfont2=\sixsy $\bullet$}\hbox{\kern-0.01em 
\textfont2=\sixsy $\bullet$}}
\hbox{$#1$\lower0.3ex \hbox{}} }}}
\def\nab#1{{\vbox{\baselineskip=0.09truein \lineskiplimit=0pt 
\moveright0.015truein\hbox{\eightpoint $\nabla$}\hbox{$#1$}}}}
\def\DL#1#2{{\vbox{\baselineskip=0.09truein \lineskiplimit=0pt 
\hbox{\eightpoint $[#1]$}\hbox{$#2$}}}}

% dot and circle for cap letters
% to have "U big dot", type {\D U}

% PC version
%\def\D#1{{\vbox{\baselineskip=0.125truein \lineskiplimit=0pt 
%\moveright0.04truein\hbox{\Largebf .}\hbox{$#1$}}}}
%\def\DD#1{{\vbox{\baselineskip=0.125truein \lineskiplimit=0pt 
%\hbox{\hbox{\Largebf .}\hbox{\Largebf .}}\hbox{$#1$}}}}

\def\D#1{{\vbox{\baselineskip=0.125truein \lineskiplimit=0pt 
\moveright0.04truein\hbox{\textfont2=\sixsy $\bullet$}\hbox{$#1$}}}}
\def\CC#1{{\vbox{\baselineskip=0.125truein \lineskiplimit=0pt 
\hbox{\hbox{\sevenrm o}\hbox{\sevenrm o}}\hbox{$#1$}}}}
\def\DD#1{{\vbox{\baselineskip=0.125truein \lineskiplimit=0pt 
\hbox{\hbox{\textfont2=\sixsy $\bullet$}\hbox{\textfont2=\sixsy 
$\bullet$}}\hbox{$#1$}}}}
% Set of the reals: This avoids using the blackboard font.
\def\real{\hbox{\rm I\kern-0.2emR}} 

% defines for accolades {}, brackets [], grouping parentheses,
% parentheses.
\def\la{\left\{}  % accolades
\def\ra{\right\}} % accolades
\def\lb{\left[}   % square brackets
\def\rb{\right]}  % square brackets
\def\lg{\left\lgroup} % grouping parentheses
\def\rg{\right\rgroup}% grouping parentheses
\def\lp{\left(}       % parentheses
\def\rp{\right)}      % parentheses

% define for double underline
\def\dunderline#1{\underline{\underline{#1}}}

% define for double overline
\def\doverline#1{\overline{\overline{#1}}}




==> smart.tex <==
%
%-------------------------------------------------------------------
% Transfer from PC to DS2100 on 16 may 90
% vql
%-------------------------------------------------------------------
%
% SMART
% This is SMART.TEX in text format, as of 87-01-21 (for TeX 2.0).
% This version is
% EASY.TEX version 1.0 by H.Partl, TU Wien
% modified and renamed to SMART.TEX by RRZN / Uni Hannover
% to avoid name conflicts
% May 1988: modified to draw framebox with thicker line (L. Vu-Quoc)
%
% SMART.TEX is a minimal macro package for TeX, using some
% ideas from The TeXbook by D.E.Knuth and LaTeX by L.Lamport.

% This macro file must not be called (\input) more than once
% inside a document.
% If a document consists of several subfiles that are input
% by a main file, each subfile should contain the sequence
% \ifundefined{chapter} \input smart \fi
% rather than a plain \input command.

\def\ifundefined#1{\expandafter\ifx\csname#1\endcsname\relax}

% AESTHETICS
%
% \sloppy     tolerate ugly line stretching
% \fussy      make it beautiful (TeX standard)
%             (These macros are taken from LaTeX)

\def\sloppy{\tolerance 2000 \hfuzz .5pt \vfuzz .5pt}
\def\fussy{\tolerance 200 \hfuzz .1pt \vfuzz .1pt}

% CONTROL SEQUENCES
%
% "o        Umlaut-o (easier to use than \"o)
% \3        scharfes s (easier to use than \ss )
% \tie      ~ (for users of Hazeltine terminals,
%           where the tilde cannot be seen)
% \today    today's date in the form  d. m. yyyy
% \date     today's date in the form yyyy-m-d

\catcode`\"=\active  \let"=\"
\let\3=\ss
\let\tie=~
\def\today{\hbox{\number\day.~\number\month.~\number\year}}
\def\date{\hbox{\number\year-\number\month-\number\day}}

% DOCUMENT LAYOUT
%
% \Narrower       is the same as \narrower, except that
%                 \displayindent is used rather than
%                 \parindent: It indents paragraphs
%                 left and right.
% \singlespacing  resets \baselineskip to \normalbaselineskip
% \halfspacing    sets \baselineskip to 1.5 character heights
% \doublespacing  sets \baselineskip to 2.0 character heights
%                 Note: If you use non-zero parskip, you
%                 should make \parskip larger, too.
%                 Recommended values are
%                 \parskip=1.5\medskipamount  for halfspacing,
%                 \parskip=2\medskipamount    for doublespacing.

\def\Narrower{\advance\leftskip by \displayindent
             \advance\rightskip by \displayindent}
\def\singlespacing{\baselineskip=\normalbaselineskip}
\def\halfspacing{\baselineskip=1.3\normalbaselineskip}
\def\doublespacing{\baselineskip=1.6\normalbaselineskip}

% \sixspacing     is spacing with \baselineskip=6pt
\def\sixspacing{\baselineskip=6truept}

% \condbreak{space}   conditional break
%                     If there is less than `space' vertical
%                     space left on the current page, then
%                     a new page is started, else do-nothing.
%                     (This is a weaker version of \filbreak.)

\def\condbreak#1{\vskip 0pt plus #1\penalty-500\vskip 0pt plus-#1}

% ENVIRONMENTS
%
% \center       the following lines until \endcenter
%               will be printed centered.
% \flushleft    the following lines until \endflushleft
%               will be printed flushed to the left.
% \flushright   the following lines until \endflushright
%               will be printed flushed to the right.
% \xxx and \endxxx must be properly paired, nesting is allowed.
% Notes: Input lines may be too long, then they will be split
% and each part will be centered or flushed, respectively.
% The macros do not say \obeyspaces, because you may need spaces
% to end command names. You can use the tie (tilde) or \quad or
% the like to produce "hard blanks" for indentation etc.
% If you don't like the \parskip before this environment,
% you should say  \vskip-\parskip  before saying \center etc.
%               (These macros use some ideas from LaTeX)

\def\center{\vskip\parskip\begingroup
            \parindent=0pt \parskip=0pt plus 1pt
            \rightskip=0pt plus 1fill \leftskip=0pt plus 1fill
            \obeylines}
\def\endcenter{\endgroup}
\def\flushleft{\vskip\parskip\begingroup
            \parindent=0pt \parskip=0pt plus 1pt
            \rightskip=0pt plus 1fill \leftskip=0pt
            \obeylines}
\def\endflushleft{\endgroup}
\def\flushright{\vskip\parskip\begingroup
            \parindent=0pt \parskip=0pt plus 1pt
            \rightskip=0pt \leftskip=0pt plus 1fill
            \obeylines}
\def\endflushright{\endgroup}

% LISTS (ITEMIZE)
%
% \itemize{width}
% \litem{label}text or \ritem{label}text
% \litem{label}text or \ritem{label}text
% ...
% \enditemize
%                   This is an extension to \item:
%                   The width of the indentation is specified
%                   in the call of \itemize, and the item label
%                   is printed left bound (by \litem) or right
%                   bound (by \ritem).
% \itemize and \enditemize must be properly paired, nesting
% with other environments (also between \litem- or \ritem-
% paragraphs) is allowed.

\def\itemize#1{\par\begingroup\parindent=#1}
\def\litem#1{\par\hang\noindent\hbox to \parindent{#1\hfil}}
\def\ritem#1{\par\hang\noindent\hbox to \parindent{\hfil#1\enspace}}
\def\enditemize{\par\endgroup\par}

% \bitem      This is a \ritem with a bullet as argument.

\def\bitem{\ritem{$\bullet$}}

% BOXES

% Box equations without boxing the equation numbers
% Boxing an equation: This macro is modified from the TeXbook, p. 331
% to surround the equation with 7pt of space on all 4 sides, and to
% begin not too far from the bottom line of the box the line that 
% follows the box; this by having \kern-8.5pt at the end of the
% macro.
%
\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern7pt\vbox{\kern7pt 
\hbox{$\displaystyle#1$}\kern7pt}\kern7pt\vrule}\hrule\kern-8.5pt}}
%
% Example of use
%   $$
%   \boxit{
%   a^2_1 {{Log (x^2 + \sqrt y)} \over {\displaystyle 1 \over z}}
%   }
%   \eqno (1.3)
%   $$

% \disbox     the following (until \enddisbox) forms a box
%             similar to that for displayed equations, but to be
%             used for texts rather than mathematics.
%             It is indented by \displayindent (left and right),
%             and it is a box, i.e. page breaks are inhibited.
%             Inside the box, all lines, environments, tables etc.
%             work as on a mini-page with the shorter line length.
% \disbox and \enddisbox must be properly paired, nesting
% with other environments and within disboxes is allowed.

\def\disbox{\vskip\parskip \hbox to\hsize\bgroup
            \hskip\displayindent \vbox\bgroup
            \advance\hsize by-2\displayindent \line{}
            \prevdepth=0pt \vskip-\parskip }
\def\enddisbox{\egroup\hss\egroup}

% \example     The following lines (until \endexample)
%              are printed flushleft with \tt font in
%              a \disbox. This is primarily intended
%              for displaying short examples of source
%              programs or the like. In contrast to verbatim,
%              TeX commands (including font changes) can be
%              used with the text.
% \example and \endexample must be properly paired, nesting
% with other environments is allowed.

\def\example{\disbox \flushleft\tt}
\def\endexample{\endflushleft\enddisbox}

% \framebox and \endframebox
%           put a frame around the text between them. The frame
%           has the full line width, the lines inside the box
%           are shortened to leave free the frame. Like hrules,
%           there is no additional space above and below the box
%           (you must use \bigskip or the like to achieve this).
%           If you do not like the \parskip before the first
%           paragraph or environment inside the box, you should
%           say  \vskip-\parskip  just after \framebox.
% \framebox and \endframebox must be properly paired, and
% all sorts of nesting are allowed (e.g. a framebox inside a disbox,
% or \center inside a framebox, or a double framebox ... ).
%
%line size has been changed to 0.8pt (L. Vu-Quoc, May 1988)

\def\framebox{\hrule height.8pt \hbox to\hsize\bgroup
              \vrule width.8pt \hskip 9.5pt
              \vbox\bgroup
              \advance\hsize by-20.2pt \line{}
              \vskip 9.5pt \nointerlineskip}
%             note: 9.5 = medskip (6.0) + interlineskip (1.5+2.0)
%                       = the blank space between \par's.
%                   20.2 = 2 * 9.5 + 2 * .8
\def\endframebox{\vskip 9.5pt \egroup \hss \vrule width.8pt
                 \egroup \hrule height.8pt}

% VERBATIM
%
% \Obeylines      same as \obeylines, but empty lines are
%                 not ignored. (used internally by verbatim mode)
%
% \verbatim       The following(!) lines of input are printed
%                 verbatim (i.e. each character as it is, including
%                 blanks and TeX's special characters, without
%                 interpretion of TeX commands) until \endverbatim.
%                 This may be used to print examples of TeX input or
%                 source programs or any data.
% \verbatim and \endverbatim must be properly paired, and they may be
% called inside some other environment.
%                 (This macro is taken from appendix D of The TeXbook)

\def\uncatcodespecials{\def\do##1{\catcode`##1=12}\dospecials\do\"}
%                     note that " is active, too.
\def\setupverbatim{\tt\Obeylines\uncatcodespecials\obeyspaces}
\def\newlinepar{~\par}
{\catcode`\^^M=\active % these lines must end with `%'
  \gdef\Obeylines{\catcode`\^^M=\active\def^^M{\newlinepar}}}
{\obeyspaces\global\let =\ }
\def\verbatim{\par\begingroup\parskip=0pt plus 1pt
              \setupverbatim\doverbatim}
{\catcode`\|=0 \catcode`\\=12
 |Obeylines|gdef|doverbatim^^M#1\endverbatim{#1|endgroup}}

% \inputverbatim{filename}
%                 The file `filename.TEX' is `input' and
%                 listed in verbatim mode.
%                 This may be used to print entire TeX input files
%                 or source program files or data files.
%                 (This macro is taken from appendix D of The TeXbook)

\def\inputverbatim#1{\par\begingroup\parskip=0pt plus 1pt
                     \setupverbatim\input#1 \endgroup}

% \verb|text|     The first character after \verb is defined as
%                 the delimiter, then the following characters
%                 are printed verbatim until the second occurrence
%                 of the delimiter. This may be used to print a short
%                 sequence of TeX commands or special characters
%                 inside a normal text.
% Caution: \verb can NOT be used inside an argument to a macro!
%                 (This macro is taken from appendix D of The TeXbook)

\def\verb{\begingroup\setupverbatim\doverb}
\def\doverb#1{\def\next##1#1{##1\endgroup}\next}

% TABLES
%
% The following is one way to extend the features of \settabs.
% You don't get ready-made macros, but you will have to define
% your own macros for each table, as follows:
%          First, chose a name `nnn' for each column of the table,
%          and define the format, width `www' and font `\ff' for
%          each column:
% \def\nnn#1{\hbox to www{\ff #1\hfil}}
%          for a left bound single-line entry,
% \def\nnn#1{\hbox to www{\hfil \ff #1}}
%          for a right bound single-line entry,
% \def\nnn#1{\hbox to www{\hfil \ff #1\hfil}}
%          for a centered single-line entry,
% \def\nnn#1{\vtop{\hsize=www \parindent=0pt \sloppy \ff #1\par}}
%          for a (short) paragraph with automatic line splitting.
%          Then, define the table (don't forget to leave space
%          between the columns, using \quad or \hskip.5cm or the like,
%          and don't exceed the line length):
% \settabs\+\nnn{x}\quad&\nnn{x}\quad& ... &\nnn{x}\cr
%          where x may be any non-blank character.
%          Now, everything is set up, and you can generate table rows
%          by
% \+\nnn{text}&\nnn{text}& ... &\nnn{text}\cr
%          (but better start a new line of input after each &)
%          and you may put anything like \medskip and/or \hrule etc.
%          between the rows.
%
% Note: If you want the table to fill the line exactly to its margins,
% the sum of the box widths plus column separations must equal \hsize.
% This can be achieved by calculating the width for one of the boxes
% by
%    \newdimen\restwidth
%    \restwidth=\hsize
%    \advance\restwidth by -sss
% where sss is the sum of the lenghts of the other boxes plus all
% column separations, and then using \restwidth as the width of that
% box.

% This is SMART10.TEX in text format, as of 1987-01-21.

% FONTS
%
% The following font names are defined:
% \large     12 point roman
% \largebf   12 point bold face
% \Large     14 point roman
% \Largebf   14 point bold face
% \small     8 point roman
% \smallit   8 point text italic

\ifnum\mag=\magstephalf

%
% for ten point font as basic font
%
%\font\large=cmr12
%\font\Large=cmr12 scaled \magstephalf
%\font\largebf=cmbx12
%\font\Largebf=cmbx12 scaled \magstephalf

%
% for twelve point font as basic font
%
 \font\large=cmr12 scaled \magstephalf
 \font\Large=cmr12 scaled \magstep1
 \font\largebf=cmbx12 scaled \magstephalf
 \font\Largebf=cmbx12 scaled \magstep1

% for use with the Stanford version of TeX, the fonts cmr## had
% been changed to amr##.  However, the font amr12 does not exist
% in this version, so use amr10 magnified.
%
%\font\large=amr10 scaled \magstephalf
%\font\Large=amr10 scaled \magstep1
%\font\largebf=ambx10 scaled \magstephalf
%\font\Largebf=ambx10 scaled \magstep1
     
\else

%
% for ten point font as basic font
%
%\font\large=cmr12
%\font\Large=cmr12 scaled \magstep1
%\font\largebf=cmbx12
%\font\Largebf=cmbx12 scaled \magstep1

%
% for twelve point font as basic font
%
 \font\large=cmr12 scaled \magstep1
 \font\Large=cmr12 scaled \magstep2
 \font\largebf=cmbx12 scaled \magstep1
 \font\Largebf=cmbx12 scaled \magstep2

% for use with the Stanford version of TeX, the fonts cmr## had
% been changed to amr##.  However, the font amr12 does not exist
% in this version, so use amr10 magnified.
%
%\font\large=amr10 scaled \magstep1
%\font\Large=amr10 scaled \magstep2
%\font\largebf=ambx10 scaled \magstep1
%\font\Largebf=ambx10 scaled \magstep2

\fi

%
% for ten point font as basic font
%
%\font\small=cmr8
%\font\smallit=cmti8

%
% for twelve point font as basic font
%
 \font\small=cmr10
 \font\smallit=cmti10

% for use with the Stanford version of TeX, the fonts cmr## had
% been changed to amr##.  However, the font amr12 does not exist
% in this version, so use amr10 magnified.
%
%\font\small=amr8
%\font\smallit=amti8


% The following skips may be used like \bigskip etc.
% They contain much stretchability, so that TeX has good chances
% to break pages where you have said \goodbreak by stretching the
% space between (not inside) chapters, sections etc.

\def\chapterskip{\vskip 1.5cm plus .75cm minus .5cm}
\def\sectionskip{\vskip 24pt plus 12pt minus 8pt}
\def\subsectionskip{\vskip 12pt plus 12pt minus 4pt}
\def\subsubsectionskip{\vskip 9pt plus 9pt minus 3pt}

% super-goodbreaks (stronger than \goodbreak, which gives
% a penalty of -500, for chapter and section breaks).

\def\Goodbreak{\par\penalty-750 }
\def\GOODbreak{\par\penalty-1000 }

% SECTION HEADINGS
%
% \chapter \section \subsection \subsubsection
%      write their argument as header to the chapter, section...
%      If you want to start a section, subsection... without any
%      head line, then you do not need to call \section...
%      The text of the heading may be longer than one line, TeX will
%      split it for you, or you may say \par to split it at a certain
%      point.
%      Depending on the current value of \toclevel, the heading
%      will also be included into a table-of-contents file.

% SPACING BETWEEN SECTIONS
%
% \endchapter \endsection \endsubsection \endsubsubsection
%     produce the (stretchable) space that is to occur between
%     two consecutive chapters, sections...
% \chapter... and \endchapter... need NOT be paired exactly.
%     You will not put \endsection after the last section of a
%     chapter just before \endchapter, and you will put
%     \endsection before the first \section header, if there
%     has been some general text (plain paragraphs) before the
%     first section header in a chapter.

% \leadersfill   fill line with dots (for table-of-contents).
%               (This macro has been taken from The Texbook.)
\def\leadersfill{\leaders\hbox to 1em{\hss.\hss}\hfill}

\outer\long\def\chapter#1{{\parindent=0pt
    \parskip=0pt \advance\baselineskip by\smallskipamount \leftskip=0pt
            \rightskip=10pt plus 1fil minus 10pt \par\largebf#1\par}
            \nobreak\smallskip\nobreak
            \expandafter\ifnum\toclevel>0
            \write\tocfile{\string\bigskip\string\goodbreak}
            \write\tocfile{\string\line{\string\rm
            {#1}\string\leadersfill \folio}}
            \fi}
\outer\def\endchapter{\par\GOODbreak\chapterskip\GOODbreak}
\outer\long\def\section#1{{\parindent=0pt
    \parskip=0pt \advance\baselineskip by\smallskipamount \leftskip=0pt
           \rightskip=10pt plus 1fil minus 10pt \par\largebf#1\par}
            \nobreak\smallskip\nobreak
           \expandafter\ifnum\toclevel>1
           \write\tocfile{\string\smallskip}
            \write\tocfile{\string\line{\string\rm
            {#1}\string\leadersfill \folio}}
           \fi}
\outer\def\endsection{\par\Goodbreak\sectionskip\Goodbreak}
\outer\long\def\subsection#1{{\parindent=0pt
    \parskip=0pt \advance\baselineskip by\smallskipamount \leftskip=0pt
            \rightskip=10pt plus 1fil minus 10pt \par\bf#1\par}
            \nobreak\smallskip\nobreak
            \expandafter\ifnum\toclevel>2
            \write\tocfile{\string\line{\string\rm
            {#1}\string\leadersfill \folio}}
            \fi}
\outer\def\endsubsection{\par\goodbreak\subsectionskip\goodbreak}
\outer\long\def\subsubsection#1{{\parindent=0pt
    \parskip=0pt \leftskip=0pt
              \rightskip=10pt plus 1fil minus 10pt \par\bf#1\par}
              \nobreak\smallskip\nobreak
              \expandafter\ifnum\toclevel>3
            \write\tocfile{\string\line{\string\rm
            {#1}\string\leadersfill \folio}}
              \fi}
\outer\def\endsubsubsection{\par\goodbreak\subsubsectionskip\goodbreak}

% TABLE OF CONTENTS
%
% \maketoc        This macro should be called at the very
%                 beginning of the document, if you want to
%                 build up a table of contents. From \maketoc
%                 on, all following chapter etc. headings will
%                 be included into a table-of-contents file
%                 (local filename ZZTOC.TEX).
%                 If you want to exclude subsubsections or
%                 subsections from the table of contents, say
%                 \toclevel=3 or \toclevel=2  after \maketoc .
%
% \printtoc       This macro should be called at the very end
%                 of the document, if you have used \maketoc
%                 before. It ends the collecting of information
%                 in file ZZTOC.TEX and prints the contents of that
%                 file, on a new page (titled `Inhaltsverzeichnis'
%                 and with roman page numbering i, ii..., so that
%                 you may move these pages to the beginning of your
%                 report before binding).
%
% Note: If you don't call \maketoc and \printtoc, there will be no
% overhead for toc generation, and file ZZTOC.TEX will not be created.

\newcount\toclevel
\toclevel=0
\newwrite\tocfile

\def\maketoc{
          \expandafter\ifnum\toclevel=0
          \openout\tocfile=zztoc
          \fi
          \toclevel=4 }

\def\printtoc{
          \vfill\eject % This also completes all \write's.
          \expandafter\ifnum\toclevel>0
          \immediate\closeout\tocfile
          \toclevel=0
          \fi
          \pageno=-1
          {\catcode`\"=12  % " has been expanded to \accent...,
                           % " is now needed for hex-constants.
          \catcode`\@=11  % @=letter is needed for PLAIN.TEX macros
                          % that have been expanded.
          \parindent=0pt
          {\largebf Inhaltsverzeichnis}\par
          \subsectionskip
          \input zztoc }}

% LAYOUT
%
% The following commands set up the layout of the document
% (paragraph shapes, aesthetics etc.)
% They CHANGE some of the definitions and settings of PLAIN.TEX,
% so that your document will look different, and various of the
% TeX commands will behave differently!

\parindent=0pt   % no indentation of first line of paragraph.
%                  Note that this affects also some macros
%                  like \item, \narrower etc. SMART_TEX contains
%                  macros that may be substitutes in this case.
\parskip=\medskipamount   % non-zero spacing between paragraphs.
%                           You may use
%                           \vskip-\parskip
%                           to remove this extra skip before a
%                           particular paragraph (e.g. before
%                           the first one in a box).
\displayindent=1cm   % indentation for displays, \disbox, \Narrower...
\overfullrule=0pt   % do not mark overfull boxes
\hoffset=0.08truein % compensate for bad page positioning

% The following are re-definitions of \makeheadline and \makefootline
% that raise the head line and lower the foot line. This will look
% better on DIN-A4 paper.
\def\makeheadline{\vbox to 0pt{\vskip-.5truein
     \line{\vbox to8.5pt{}\the\headline}\vss}\nointerlineskip}
\def\makefootline{\baselineskip=.5truein \line{\the\footline}}

% The following macros may be called to change the page layout:
% \noheadlines     disables head lines and moves up the beginning
%                  of the normal text per page by .5 inch.
% \nofootlines     disables foot lines and page numbers, and moves
%                  down the end of the normal text per page by .5 inch.
% These macros should be called only once and only at the very beginning
% of the document.
\def\noheadlines{\def\makeheadline{}
                 \advance\voffset by-.5truein \advance\vsize by.5truein}
\def\nofootlines{\def\makefootline{}\advance\vsize by.5truein}

% \Footnote   a better version of \footnote,
%             with internal and constant settings
%             of parindent, parskip and font.

\def\Footnote#1#2{{\parindent=1cm \baselineskip=11pt
    \footnote{#1}{\vrule height10.5pt width0pt \small #2}}}

% \note       automatically numbered footnotes (taken from the TeXbook,
%             exercise 15.12

\newcount\notenumber
\def\clearnotenumber{\notenumber=0}
\def\note{\advance\notenumber by 1
    \Footnote{$^{\the\notenumber}$}}

